The Potential Impact of AI Innovations on U.S. Occupations

An occupation is comprised of interconnected tasks, and it is these tasks, not occupations themselves, that are affected by AI. To evaluate how tasks may be impacted, previous approaches utilized manual annotations or coarse-grained matching. Leveraging recent advancements in machine learning, we replace coarse-grained matching with more precise deep learning approaches. Introducing the AI Impact (AII) measure, we employ Deep Learning Natural Language Processing to automatically identify AI patents that may impact various occupational tasks at scale. Our methodology relies on a comprehensive dataset of 17,879 task descriptions and quantifies AI's potential impact through analysis of 24,758 AI patents filed with the United States Patent and Trademark Office (USPTO) between 2015 and 2022. Our results reveal that some occupations will potentially be impacted, and that impact is intricately linked to specific skills. These include not only routine tasks (codified as a series of steps), as previously thought, but also non-routine ones (e.g., diagnosing health conditions, programming computers, and tracking flight routes). However, AI's impact on labour is limited by the fact that some of the occupations affected are augmented rather than replaced (e.g., neurologists, software engineers, air traffic controllers), and the sectors affected are experiencing labour shortages (e.g., IT, Healthcare, Transport).

==> tables/2022/counties.tex <==
\begin{table*}[t!]
    \centering
    \caption{Most- and least-impacted counties. The county-level AII is calculated as the employment-weighted average of sector-level AII scores, weighted by the importance of each economic sector in the county. For each county, we also report the economic diversity (higher values indicate greater diversity) and the predominant employment sector. The economic diversity values for all counties shown are less than 2.8, which is the cutoff for the 1\textsuperscript{st} quartile. This indicates that these counties have relatively low economic diversity, with their workforce concentrated in just a few sectors. }
    \scalebox{0.95}{
    \begin{tabular}{|c|lcl|lcl|}
    \hline
    \textbf{Rank} & \textbf{Most-impacted} & \textbf{\shortstack[c]{Economic \\ Diversity}} & \textbf{Most Prevalent Sector} & \textbf{Least-impacted} & \textbf{\shortstack[c]{Economic \\ Diversity}} & \textbf{Most Prevalent Sector} \\
    \hline
    1 & Buffalo County, SD & 1.65 & Healthcare & Moore County, TN & 1.47 & Education \\
    2 & Robertson County, KY & 1.74 & Healthcare & Arthur County, NE & 1.02 & Education \\
    3 & Aleutians East Borough, AK & 0.78 & Manufacturing & Calhoun County, IL & 2.29 & Education \\
    4 & Delta County, TX & 2.26 & Healthcare & Denali Borough, AK & 1.71 & Accommodation and food services \\
    5 & Cumberland County, KY & 2.37 & Healthcare & Glascock County, GA & 1.16 & Education \\
    6 & Metcalfe County, KY & 2.71 & Healthcare & McPherson County, NE & 1.08 & Education \\
    7 & Cameron County, PA & 1.77 & Manufacturing & Piute County, UT & 1.66 & Education \\
    8 & Hardin County, IL & 2.32 & Healthcare & Banner County, NE & 1.27 & Education \\
    9 & District of Columbia & 0.96 & Administrative & Loup County, NE & 1.22 & Education \\
    10 & Miller County, GA & 2.39 & Healthcare & Long County, GA & 1.83 & Education \\
    11 & Starr County, TX & 2.34 & Healthcare & Oldham County, TX & 1.82 & Education \\
    12 & Evangeline Parish, LA & 2.73 & Healthcare & Elk County, KS & 1.99 & Education \\
    13 & Saluda County, SC & 2.37 & Manufacturing & Love County, OK & 2.79 & Accommodation and food services \\
    14 & Duval County, TX & 2.47 & Healthcare & Gilpin County, CO & 1.95 & Accommodation and food services \\
    15 & Hancock County, KY & 2.10 & Manufacturing & Williamsburg City, VA & 2.86 & Education \\
    16 & Franklin County, TX & 2.69 & Healthcare & Tunica County, MS & 2.11 & Accommodation and food services \\
    17 & Todd County, SD & 2.05 & Healthcare & Frontier County, NE & 2.48 & Education \\
    18 & Storey County, NV & 2.45 & Manufacturing & Garfield County, UT & 2.40 & Accommodation and food services \\
    19 & Elkhart County, IN & 2.63 & Manufacturing & Wheeler County, GA & 1.56 & Education \\
    20 & Red River County, TX & 3.21 & Healthcare & Harding County, NM & 1.83 & Education \\
    \hline
    \end{tabular}
    }
    \label{tab:counties_impact}
\end{table*}

==> tables/aii.tex <==
\aboverulesep=0ex
\belowrulesep=0ex

\begin{table*}[t!]
    \centering
    \caption{20 most- and least-impacted occupations ranked by the AII (Artificial Intelligence Impact) measure.}
    \label{tab:job_aii}
    \scalebox{0.8}{
    \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Rank} & \textbf{Most-impacted} & \textbf{Least-impacted} \\
    \hline
    1 & Cardiovascular Technologists and Technicians & Pile-Driver Operators \\
    \hdashline
    2 & Orthodontists & Graders and Sorters, Agricultural Products \\
    \hdashline
    3 & Medical Records and Health Information Technicians & Floor Sanders and Finishers \\
    \hdashline
    4 & Numerical Tool and Process Control Programmers & Aircraft Cargo Handling Supervisors \\
    \hdashline
    5 & Multi-Media Artists and Animators & Dredge Operators \\
    \hdashline
    6 & Magnetic Resonance Imaging Technologists & Insurance Appraisers, Auto Damage \\
    \hdashline
    7 & Nuclear Medicine Technologists & Insurance Underwriters \\
    \hdashline
    8 & Software Developers, Applications & Reinforcing Iron and Rebar Workers \\
    \hdashline
    9 & Electro-Mechanical Technicians & Farm Labor Contractors \\
    \hdashline
    10 & Industrial Truck and Tractor Operators & Water and Liquid Waste Treatment Plant and System Operators \\
    \hdashline
    11 & Sound Engineering Technicians & Animal Scientists \\
    \hdashline
    12 & Computer Programmers & Brokerage Clerks \\
    \hdashline
    13 & Life, Physical, and Social Science Technicians, All Other & Insulation Workers, Floor, Ceiling, and Wall \\
    \hdashline
    14 & Earth Drillers, Except Oil and Gas & Locomotive Firers \\
    \hdashline
    15 & Medical Transcriptionists & Management Analysts \\
    \hdashline
    16 & Grinding, Lapping, Polishing, and Buffing Machine Tool Setters, Operators, and Tenders, Metal and Plastic & Podiatrists \\
    \hdashline
    17 & Airline Pilots, Copilots, and Flight Engineers & Cooks, Short Order \\
    \hdashline
    18 & Physical Scientists, All Other & Shipping, Receiving, and Traffic Clerks \\
    \hdashline
    19 & Computer-Controlled Machine Tool Operators, Metal and Plastic & Helpers--Painters, Paperhangers, Plasterers, and Stucco Masons \\
    \hdashline
    20 & Biomedical Engineers & Team Assemblers \\
    \hline
    \end{tabular}
    }
\end{table*}

==> tables/aug/aii.tex <==
\aboverulesep=0ex
\belowrulesep=0ex

\begin{table*}[t!]
    \centering
    \caption{20 most- and least-impacted occupations ranked by AII (augmentation) measure.}
    \label{tab:job_aii}
    \scalebox{0.8}{
    \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Rank} & \textbf{Most-impacted} & \textbf{Least-impacted} \\
    \hline
    1 & Magnetic Resonance Imaging Technologists & Human Resources Specialists \\
    \hdashline
    2 & Hearing Aid Specialists & Credit Counselors \\
    \hdashline
    3 & Electrical and Electronics Repairers, Commercial and Industrial Equipment & Agricultural Technicians \\
    \hdashline
    4 & Electromechanical Equipment Assemblers & Special Education Teachers, Secondary School \\
    \hdashline
    5 & Computer Numerically Controlled Tool Operators & Adapted Physical Education Specialists \\
    \hdashline
    6 & Electrical and Electronic Equipment Assemblers & Art Directors \\
    \hdashline
    7 & Fabric and Apparel Patternmakers & Fine Artists, Including Painters, Sculptors, and Illustrators \\
    \hdashline
    8 & Computer Numerically Controlled Tool Programmers & Dentists, General \\
    \hdashline
    9 & Cardiovascular Technologists and Technicians & Surgical Assistants \\
    \hdashline
    10 & Wind Turbine Service Technicians & Speech-Language Pathology Assistants \\
    \hdashline
    11 & Diagnostic Medical Sonographers & Security Guards \\
    \hdashline
    12 & Cartographers and Photogrammetrists & Sales Representatives, Wholesale and Manufacturing, Technical and Scientific Products \\
    \hdashline
    13 & Food Science Technicians & Sales Representatives, Wholesale and Manufacturing, Except Technical and Scientific Products \\
    \hdashline
    14 & Orthodontists & Models \\
    \hdashline
    15 & Prosthodontists & Real Estate Brokers \\
    \hdashline
    16 & Radiologic Technologists and Technicians & Carpet Installers \\
    \hdashline
    17 & Electrical and Electronics Drafters & Drywall and Ceiling Tile Installers \\
    \hdashline
    18 & Audiologists & Insulation Workers, Floor, Ceiling, and Wall \\
    \hdashline
    19 & Ophthalmic Medical Technicians & Paperhangers \\
    \hdashline
    20 & Desktop Publishers & Helpers--Carpenters \\
    \hline
    \end{tabular}
    }
\end{table*}

==> tables/aug/counties.tex <==
\begin{table*}[t!]
    \centering
    \caption{Most- and least-impacted counties by AII (augmentation). The county-level AII is calculated as the employment-weighted average of sector-level AII scores, weighted by the importance of each economic sector in the county. For each county, we also report the economic diversity (higher values indicate greater diversity) and the predominant employment sector. The economic diversity values for all counties shown are less than 2.8, which is the cutoff for the 1\textsuperscript{st} quartile. This indicates that these counties have relatively low economic diversity, with their workforce concentrated in just a few sectors. }
    \scalebox{0.95}{
    \begin{tabular}{|c|lcl|lcl|}
    \hline
    \textbf{Rank} & \textbf{Most-impacted} & \textbf{\shortstack[c]{Economic \\ Diversity}} & \textbf{Most Prevalent Sector} & \textbf{Least-impacted} & \textbf{\shortstack[c]{Economic \\ Diversity}} & \textbf{Most Prevalent Sector} \\
    \hline
    1 & Loving County, Texas & 1.05 & Mining & Denali Borough, Alaska & 1.71 & Accommodation and food services \\
    2 & Irion County, Texas & 1.66 & Mining & Tunica County, Mississippi & 2.11 & Accommodation and food services \\
    3 & Shackelford County, Texas & 2.02 & Mining & Keweenaw County, Michigan & 2.13 & Accommodation and food services \\
    4 & McMullen County, Texas & 1.73 & Mining & Gilpin County, Colorado & 1.95 & Accommodation and food services \\
    5 & Reagan County, Texas & 1.88 & Mining & Garfield County, Utah & 2.40 & Accommodation and food services \\
    6 & Dewey County, Oklahoma & 2.56 & Mining & Mineral County, Colorado & 2.42 & Public administration \\
    7 & Winkler County, Texas & 2.33 & Mining & Lake of the Woods County, Minnesota & 2.57 & Accommodation and food services \\
    8 & North Slope Borough, Alaska & 2.22 & Mining & Arthur County, Nebraska & 1.02 & Education services \\
    9 & Upton County, Texas & 2.11 & Mining & Moore County, Tennessee & 1.47 & Education services \\
    10 & Dimmit County, Texas & 2.73 & Mining & Mahnomen County, Minnesota & 2.28 & Accommodation and food services \\
    11 & Hemphill County, Texas & 2.98 & Mining & Stanley County, South Dakota & 2.63 & Accommodation and food services \\
    12 & Crane County, Texas & 2.91 & Mining & Mackinac County, Michigan & 2.60 & Accommodation and food services \\
    13 & Karnes County, Texas & 3.19 & Mining & Calhoun County, Illinois & 2.29 & Education services \\
    14 & Ochiltree County, Texas & 3.14 & Mining & Piute County, Utah & 1.66 & Education services \\
    15 & Claiborne Parish, Louisiana & 3.03 & Mining & Loup County, Nebraska & 1.22 & Education services \\
    16 & Duval County, Texas & 2.47 & Health care and social assistance & McPherson County, Nebraska & 1.08 & Education services \\
    17 & Jack County, Texas & 3.05 & Mining & Mono County, California & 2.66 & Accommodation and food services \\
    18 & Glasscock County, Texas & 1.60 & Agriculture, forestry, fishing and hunting & San Juan County, Colorado & 2.50 & Accommodation and food services \\
    19 & Hockley County, Texas & 3.10 & Mining & Glascock County, Georgia & 1.16 & Education services \\
    20 & Midland County, Texas & 3.58 & Mining & Rich County, Utah & 2.97 & Accommodation and food services \\
    \hline
    \end{tabular}
    }
    \label{tab:counties_impact}
\end{table*}

==> tables/counties.tex <==
\begin{table*}[t!]
    \centering
    \caption{Most- and least-impacted counties. The county-level AII is calculated as the employment-weighted average of sector-level AII scores, weighted by the importance of each economic sector in the county. For each county, we also report the economic diversity (higher values indicate greater diversity) and the predominant employment sector. The economic diversity values for all counties shown are less than 2.8, which is the cutoff for the 1\textsuperscript{st} quartile. This indicates that these counties have relatively low economic diversity, with their workforce concentrated in just a few sectors. }
    \scalebox{0.95}{
    \begin{tabular}{|c|lcl|lcl|}
    \hline
    \textbf{Rank} & \textbf{Most-impacted} & \textbf{\shortstack[c]{Economic \\ Diversity}} & \textbf{Most Prevalent Sector} & \textbf{Least-impacted} & \textbf{\shortstack[c]{Economic \\ Diversity}} & \textbf{Most Prevalent Sector} \\
    \hline
    1 & Issaquena County, MS & 0.54 & Healthcare & Wallace County, KS & 1.55 & Finance and insurance \\
    2 & Petroleum County, MT & 1.30 & Healthcare & Hinsdale County, CO & 1.55 & Construction \\
    3 & Buffalo County, SD & 1.46 & Healthcare & Twiggs County, GA & 1.00 & Education \\
    4 & Macon County, AL & 1.67 & Healthcare & Heard County, GA & 1.18 & Education \\
    5 & Jefferson County, MS & 1.79 & Healthcare & Graham County, NC & 2.39 & Education \\
    6 & Starr County, TX & 1.74 & Healthcare & Garfield County, MT & 1.24 & Education \\
    7 & Iron County, MO & 1.80 & Healthcare & Storey County, NV & 1.00 & Transportation  \\
    8 & Metcalfe County, KY & 1.99 & Healthcare & Phillips County, MT & 2.64 & Education \\
    9 & Calhoun County, AR & 0.55 & Manufacturing & Clark County, ID & 1.07 & Education \\
    10 & Ripley County, MO & 2.27 & Healthcare & Ottawa County, KS & 2.51 & Finance and insurance \\
    11 & Galax City, VA & 1.94 & Healthcare & Zavala County, TX & 1.39 & Education \\
    12 & Dillingham Census Area, AK & 0.90 & Manufacturing & McPherson County, SD & 1.29 & Education \\
    13 & Evangeline Parish, Louisiana & 2.35 & Healthcare & Red Lake County, MN & 2.46 & Education \\
    14 & Aleutians East Borough, AK & 0.69 & Manufacturing & Judith Basin County, MT & 1.99 & Education \\
    15 & Franklin City, VA & 2.37 & Healthcare & Gates County, NC & 1.99 & Education \\
    16 & Sherman County, NE & 2.20 & Healthcare & Calhoun County, IL & 2.11 & Education \\
    17 & Reynolds County, MO & 2.33 & Manufacturing & Kingman County, KS & 2.85 & Education \\
    18 & Borden County, TX & 1.87 & Healthcare & Clay County, TX & 1.65 & Education \\
    19 & Todd County, SD & 1.57 & Healthcare & Denali Borough, AK & 0.91 & Accommodation and food services \\
    20 & Wayne County, KY & 2.14 & Manufacturing & Lincoln County, KS & 2.25 & Education \\
    \hline
    \end{tabular}
    }
    \label{tab:counties_impact}
\end{table*}

==> tables/keywords.tex <==
\begin{table}[h!]
    \centering
    \caption{Number of patents based on keywords.}
    \label{tab:keywords}
    \begin{tabular}{|l|c|}
    \hline
    Keywords & Number of patents \\
    \hline
    machine learning & 6084 \\
    \hdashline
    neural network & 4197 \\
    \hdashline
    artificial intelligence & 1210 \\ 
    \hdashline
    deep learning & 810 \\
    \hdashline
    natural language processing & 758 \\
    \hdashline
    planning & 595 \\
    \hdashline
    reinforcement learning & 232 \\
    \hdashline
    computer vision & 211 \\
    \hdashline
    speech processing & 73 \\
    \hdashline
    predictive analytics & 47 \\
    \hdashline
    robotics & 35 \\
    \hdashline
    knowledge representation & 21 \\
    \hdashline
    control methods & 15 \\    
    \hline
    \end{tabular}
\end{table}

==> tables/task-patent-jobs.tex <==
\begin{table*}[t!]
    \centering
     \caption{The most-impacted occupations based on AII scores. Each occupation's score is calculated as the number of impacted tasks divided by the total number of tasks for that occupation. For each occupation, a task-patent pair is presented, corresponding to the most impacted task by the patent (i.e., the patent with the highest similarity score to the task) which is determined by calculating the textual similarity between the task's description and a patent's title plus abstract. }
    \label{tab:job_tasks_patents}
    \scalebox{0.7}{
    \begin{tabular}{|c|p{4cm}p{2.1cm}p{6cm}p{4cm}ccc|c|}
        \hline
        \textbf{Rank} & \textbf{Occupation} & \textbf{Sector} & \textbf{Task} & \textbf{Patent} & \textbf{Similarity} & \textbf{\shortstack[c]{\# Impacted \\ Tasks}} & \textbf{\shortstack[c]{Total \\ Tasks}} & \textbf{AII} \\
        \hline
        1 & Cardiovascular Technologists and Technicians & Healthcare & Observe gauges, recorder, and video screens [...] during imaging of cardiovascular system. & Automated analysis of vasculature in coronary angiograms & 0.8753 & 15 & 25 & 0.60 \\
        \hdashline
        2 & Orthodontists & Healthcare & Study diagnostic records, such as medical or dental histories [...] to develop patient treatment plans. & Patient-Specific Therapy Planning Support Using Patient Matching & 0.8460 & 6 & 10 & 0.60 \\
        \hdashline
        3 & Medical Records and Health Information Technicians & Healthcare & Plan, develop, maintain, or operate a variety of health record indexes [...] & Dynamic health record problem list & 0.8350 & 10 & 20 & 0.50 \\
        \hdashline
        4 & Numerical Tool and Process Control Programmers & Manufacturing & Determine the sequence of machine operations, [...] & Methods and apparatuses for cutter path planning and for workpiece machining & 0.8376 & 8 & 16 & 0.50 \\
        \hdashline
        5 & Multi-Media Artists and Animators & Information & Create pen-and-paper images to be [...] animated by computer. & Line drawing generation & 0.8396 & 7 & 14 & 0.50 \\
        \hdashline
        6 & Magnetic Resonance Imaging Technologists & Healthcare & Operate optical systems to capture dynamic magnetic resonance imaging (MRI) images [...] & MRI system and method using neural network for detection of patient motion & 0.8615 & 11 & 23 & 0.48 \\
        \hdashline
        7 & Nuclear Medicine Technologists & Healthcare & Gather information on patients' illnesses and medical history to guide the choice of diagnostic procedures for therapy. & Patient-Specific Therapy Planning Support Using Patient Matching & 0.8630 & 8 & 17 & 0.47 \\
        \hdashline
        8 & Software Developers, Applications & Information & Design [...] mathematical models to predict and measure outcome and consequences of design. & Adaptive predictive analytics for design modification requests & 0.8295 & 7 & 15 & 0.47 \\
        \hdashline
        9 & Electro-Mechanical Technicians & Manufacturing & Train robots, using artificial intelligence software or interactive training techniques, [...] & Architectures, systems and methods for program defined entertainment state system, [...] & 0.8535 & 16 & 35 & 0.46 \\
        \hdashline
        10 & Industrial Truck and Tractor Operators & Manufacturing & Move controls to drive gasoline- or electric-powered trucks, cars, or tractors and transport materials between loading, processing, and storage areas. & Autonomous Truck Unloading for Mining and Construction Applications & 0.8301 & 5 & 11 & 0.45 \\
        \hdashline
        11 & Sound Engineering Technicians & Arts and entertainment & Record speech, music, and other sounds on recording media, using recording equipment. & Media capture and process system & 0.8293 & 6 & 14 & 0.43 \\
        \hdashline
        12 & Computer Programmers & Information & Prepare detailed workflow charts and diagrams [...] & System and method for generating flowchart from a text document using natural language processing & 0.8443 & 7 & 17 & 0.41 \\
        \hdashline
        13 & Life, Physical, and Social Science Technicians, All Other & Scientific and technical services & Adjust remotely sensed images for optimum presentation [...] & Smart imaging using artificial intelligence & 0.8374 & 27 & 67 & 0.40 \\
        \hdashline
        14 & Earth Drillers, Except Oil and Gas & Construction & Operate water-well drilling rigs and other equipment [...] & Systems and methods for oilfield drilling operations using computer vision & 0.8280 & 12 & 30 & 0.40 \\
        \hdashline
        15 & Medical Transcriptionists & Healthcare & Transcribe dictation for a variety of medical reports [...] & Methods for improving natural language processing [...] for automated generation of a clinical summarization report [...] & 0.8367 & 6 & 15 & 0.40 \\
        \hdashline
        16 & Grinding, Lapping, Polishing, and Buffing Machine Tool Setters, Operators, and Tenders, Metal and Plastic & Manufacturing & Move machine controls to index workpieces, and to adjust machines for pre-selected operational settings. & Motor control apparatus & 0.8218 & 7 & 18 & 0.39 \\
        \hdashline
        17 & Airline Pilots, Copilots, and Flight Engineers & Transportation & Steer aircraft along planned routes, using autopilot and flight management computers. & Cumulative model for scheduling and resource allocation for airline operations & 0.8367 & 10 & 26 & 0.38 \\
        \hdashline
        18 & Physical Scientists, All Other & Scientific and technical services & Develop automated routines to correct for the presence of image distorting artifacts, such as ground vegetation. & Detection and Management of Target Vegetation Using Machine Vision & 0.8345 & 9 & 24 & 0.38 \\
        \hdashline
        19 & Computer-Controlled Machine Tool Operators, Metal and Plastic & Manufacturing & Implement changes to machine programs, and enter new specifications, using computers. & Registering collaborative configuration changes of a network element in a blockchain ledger & 0.8370 & 10 & 27 & 0.37 \\
        \hdashline
        20 & Biomedical Engineers & Healthcare & Diagnose and interpret bioelectric data, using signal processing techniques. & Electrocardiogram Device and Methods & 0.8622 & 7 & 19 & 0.37 \\
        \hline
    \end{tabular}
    }
\end{table*}

==> tables/task-patent-sectors.tex <==
\begin{table*}[htbp]
    \centering
    \caption{For each industry sector, the most representative occupations are selected. A task-patent pair is presented, corresponding to the task most impacted by the patent in the selected occupations. This is determined by calculating the similarity of the SBERT embeddings between the task's description and a patent's abstract. The number of tasks and occupations impacted by a patent is presented, and the total number of tasks and occupations within each sector is presented in parentheses. \todo{comment in the body about the specificity of the patents. one patent might be very specific for an occupation. change the order of columns}}
    \label{tab:sectors_pantents_tasks}

    % TODO: order columns: Sector, #Most Impacted Tasks in Sector by Patent, #Most Impacted Occupations in Sector  by Patent, Example Task, Patent
    
    \scalebox{0.6}{
    \begin{tabular}{p{4cm}p{6cm}p{5cm}cc}
        \toprule
        \textbf{Sector} & \textbf{Task} & \textbf{Patent} & \textbf{{\shortstack[c]{\# Tasks Impacted \\by Patent}}}  & \textbf{{\shortstack[c]{\# Occupations Impacted \\by Patent}}}\\
        \midrule
        Health care and social assistance & Interpret images using computer-aided detection or diagnosis systems. & Methods and systems for automatically analyzing clinical images using rules and image analytics & 1 (1459) & 1 (70) \\
        \hdashline
        Information & Test circuits and components of malfunctioning telecommunications equipment to isolate sources of malfunctions, using test meters, circuit diagrams, polarity probes, and other hand tools. & Telecommunications network troubleshooting systems & 16 (314) & 13 (13) \\
        \hdashline
        Professional, Scientific and Technical Services & Analyze aerial photographs to detect and interpret significant military, industrial, resource, or topographical data. & Determining stockpile volume based on digital aerial images and three-dimensional representations of a site & 1 (329) & 1 (15) \\
        \hdashline
        Manufacturing & Examine chemical or biological samples to identify cell structures or to locate bacteria or extraneous material, using a microscope. & Microscopy method, microscope and computer program with verification algorithm for image processing results & 13 (2260) & 12 (109) \\
        \hdashline
        Utilities & Start or restart wind turbine generator systems to ensure proper operations. & Methods and systems for alleviating loads in off-shore wind turbines & 22 (353) & 4 (14) \\
        \hdashline
        Transportation and warehousing & Obtain and review data such as load weights, fuel supplies, weather conditions, and flight schedules to determine flight plans and identify needed changes. & Aircraft flight planning apparatus and method & 14 (612) & 6 (26) \\
        \hdashline
        Administrative and support and waste management and remediation services & Operate underwater video, sonar, recording, or related equipment to investigate underwater structures or marine life. & Underwater camera and water quality monitoring system & 5 (174) & 2 (10) \\
        \hdashline
        Agriculture, forestry, fishing and hunting & Manipulate controls to set, activate, and adjust mechanisms on machinery. & Motor control apparatus & 36 (181) & 32 (8) \\
        \hdashline
        Wholesale trade & Test components or circuits of faulty equipment to locate defects, using oscilloscopes, signal generators, ammeters, voltmeters, or special diagnostic software programs. & Machine learning-based fault detection system & 2 (71) & 2 (4) \\
        \hdashline
        Mining & Simulate reservoir performance for different recovery techniques, using computer models. & System and method for using an artificial neural network to simulate pipe hydraulics in a reservoir simulator & 1 (118) & 1 (7) \\
        \hdashline
        Retail trade & Rebuild, repair, or test automotive fuel injection units. & Fuel injection system and method for a vehicle propulsion system & 3 (473) & 1 (22) \\
        \hdashline
        Arts, entertainment, and recreation & Create sketches, profiles, or likenesses of posed subjects or photographs, using any combination of freehand drawing, mechanical assembly kits, and computer imaging. & Sketch Completion Using Machine Learning & 5 (386) & 5 (19) \\
        \hdashline
        Public administration & Measure and record the speed of vehicular traffic, using electrical timing devices or radar equipment. & System and method for detecting, tracking and estimating the speed of vehicles from a mobile platform & 1 (1002) & 1 (42) \\
        \hdashline
        Accommodation and food services & Plan and develop programs, agendas, budgets, and services according to customer requirements. & System and method for custom-fitting services to consumer requirements & 99 (337) & 65 (17) \\
        \hdashline
        Other services, except public administration & Monitor equipment operation to detect malfunctions. & System and method for automated fault diagnosis and prognosis for rotating equipment & 47 (470) & 37 (22) \\
        \hdashline
        Construction & Polish surface, using polishing or surfacing machine. & Monitoring of polishing pad texture in chemical mechanical polishing & 92 (736) & 50 (36) \\
        \hdashline
        Education services & Prepare, store, and retrieve classification and catalog information, lecture notes, or other information related to stored documents, using computers. & Automatic document classification via content analysis at storage time & 5 (2022) & 4 (75) \\
        \hdashline
        Real estate and rental and leasing & Generate lists of properties for sale, their locations, descriptions, and available financing options, using computers. & System and method for generating a probability score indicative of a probability that an owner will sell a real estate property & 12 (35) & 6 (2) \\
        \hdashline
        Finance and insurance & Explain, promote, or sell products or services, such as travelers' checks, savings bonds, money orders, and cashier's checks, using computerized information about customers to tailor recommendations. & Computer implemented system and method for customer profiling using micro-conversions via machine learning & 15 (297) & 10 (14) \\
        \hdashline
        \bottomrule
    \end{tabular}
    }
\end{table*}
